Deep-Learning based Reconstruction of the Shower Maximum $X_{\mathrm{max}}$ using the Water-Cherenkov Detectors of the Pierre Auger Observatory

The atmospheric depth of the air shower maximum $X_{\mathrm{max}}$ is an observable commonly used for the determination of the nuclear mass composition of ultra-high energy cosmic rays. Direct measurements of $X_{\mathrm{max}}$ are performed using observations of the longitudinal shower development with fluorescence telescopes. At the same time, several methods have been proposed for an indirect estimation of $X_{\mathrm{max}}$ from the characteristics of the shower particles registered with surface detector arrays. In this paper, we present a deep neural network (DNN) for the estimation of $X_{\mathrm{max}}$. The reconstruction relies on the signals induced by shower particles in the ground based water-Cherenkov detectors of the Pierre Auger Observatory. The network architecture features recurrent long short-term memory layers to process the temporal structure of signals and hexagonal convolutions to exploit the symmetry of the surface detector array. We evaluate the performance of the network using air showers simulated with three different hadronic interaction models. Thereafter, we account for long-term detector effects and calibrate the reconstructed $X_{\mathrm{max}}$ using fluorescence measurements. Finally, we show that the event-by-event resolution in the reconstruction of the shower maximum improves with increasing shower energy and reaches less than $25~\mathrm{g/cm^{2}}$ at energies above $2\times 10^{19}~\mathrm{eV}$.

==> Makefile <==
# Makefile for building latex documents (c) Darko Veberic
# $Id: Makefile 1342 2019-01-29 17:20:57Z darko $

USEPDFLATEX := 1
USEBIBTEX := 0

TEXFILES := $(shell grep -le '^\s*\\document\(class\|style\)' *.tex)
TARGETS := $(basename $(TEXFILES))
DEPENDENCIES := $(wildcard *.sty *.bib figs/*) $(filter-out $(TEXFILES), $(wildcard *.tex))

##########################################################
SHELL := /bin/bash
PDFS := $(addsuffix .pdf, $(TARGETS))

ifeq (, $(shell which latexmk))
  LATEX := $(if $(filter 1, $(USEPDFLATEX)), pdflatex, latex)
  # 30=black 31=red 32=green 33=yellow 34=blue 35=magenta 36=cyan 37=white 0=cancel
  COLORIZE := awk 'BEGIN{ec="\033[31;1m";wc="\033[34;1m";cc="\033[0m"}/Rerun /||/rerunfilecheck[^.]/{e=e$$0"\n";print ec""$$0""cc;next}/^LaTeX Warning:/||/natbib Warning:/{w=w$$0"\n";print wc""$$0""cc;next}{print}END{if(w||e)print "\n"ec"Warning/error summary:"cc"\n"wc""w""cc;if(e){print ec""e""cc;exit 1}}'
  define basic_latex_rule
    for i in 1 2 3 ; do $(LATEX) $< | $(COLORIZE) && break ; done
  endef
  ifeq ($(USEBIBTEX), 1)
    define latex_rule
      $(LATEX) $< ; bibtex $*
      $(call basic_latex_rule)
    endef
  else
    define latex_rule
      $(call basic_latex_rule)
    endef
  endif
else
  define latex_rule
    latexmk $(if $(filter 1, $(USEPDFLATEX)), -pdf, ) $<
  endef
endif

.PHONY: all clean

all: $(PDFS)

# dependencies
$(PDFS): $(DEPENDENCIES)

clean:
	- $(RM) *{.tex~,.dvi,.log,.aux,.toc,.nav,.out,.snm,.bbl,.blg,.spl,.lof,Notes.bib,.maf,.fff,.lot,.ttt,.bcf,.run.xml,.fdb_latexmk,.fls,.synctex.gz}
	- for f in $(TARGETS) ; do $(RM) $$f{.ps,.pdf} ; done

# general rules
ifeq ($(USEPDFLATEX), 1)
%.pdf: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.ps: %.pdf
	pdf2ps $<
else
%.dvi: %.tex $(DEPENDENCIES)
	$(call latex_rule)

%.pdf: %.dvi
	dvipdf $<

%.ps: %.dvi
	dvips $< -o
endif

# embed pdf fonts
%.embedded_fonts.pdf: %.pdf
	gs -dSAFER -dNOPLATFONTS -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sPAPERSIZE=a4 -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sOutputFile=$@ -f $<

